QuantProb: Generalizing Probabilities along with Predictions for a Pre-trained Classifier

Quantification of Uncertainty in predictions is a challenging problem. In the classification settings, although deep learning based models generalize well, class probabilities often lack reliability. Calibration errors are used to quantify uncertainty, and several methods exist to minimize calibration error. We argue that between the choice of having a minimum calibration error on original distribution which increases across distortions or having a (possibly slightly higher) calibration error which is constant across distortions, we prefer the latter We hypothesize that the reason for unreliability of deep networks is - The way neural networks are currently trained, the probabilities do not generalize across small distortions. We observe that quantile based approaches can potentially solve this problem. We propose an innovative approach to decouple the construction of quantile representations from the loss function allowing us to compute quantile based probabilities without disturbing the original network. We achieve this by establishing a novel duality property between quantiles and probabilities, and an ability to obtain quantile probabilities from any pre-trained classifier. While post-hoc calibration techniques successfully minimize calibration errors, they do not preserve robustness to distortions. We show that, Quantile probabilities (QuantProb), obtained from Quantile representations, preserve the calibration errors across distortions, since quantile probabilities generalize better than the naive Softmax probabilities.

==> Table_Neurips_Rebuttal.tex <==
\begin{table}
    \caption{Comparison of Quantile-Representations with baseline for OOD Detection.The entries are represented as \textsc{QuantileMaxProb}/\textsc{BaselineMaxLogit}/\textsc{Difference}.} Note that the article - ``Open-Set Recognition: A Good Closed-Set Classifier is All You Need'' (ICLR 2022) shows that with ``good'' training, the Maximum Logit Score achieves state-of-art. Hence this is considered as a baseline. 
    \label{table:1}
    \begin{center}
    \begin{small}

\begin{tabular}{lllll}
\toprule
 &  & AUROC & TNR-TPR95 & Det.Acc \\
Model/ID & OOD &  &  &  \\
\midrule
\multirow[t]{5}{*}{ResNet34/CIFAR10} & Imagenet(C) & \textbf{92.68}/92.27/(0.41) & \textbf{63.88}/57.31/(6.57) & \textbf{86.26}/85.70/(0.56) \\
 & Imagenet(R) & \textbf{92.13}/91.47/(0.65) & \textbf{61.44}/53.37/(8.07) & \textbf{85.69}/84.90/(0.80) \\
 & LSUN(C) & 92.51/\textbf{93.53}/(-1.02) & \textbf{64.00}/61.77/(2.23) & 86.92/\textbf{87.24}/(-0.32) \\
 & LSUN(R) & \textbf{94.83}/91.55/(3.28) & \textbf{71.87}/55.07/(16.80) & \textbf{88.96}/85.20/(3.75) \\
 & iSUN & \textbf{94.17}/91.76/(2.41) & \textbf{70.36}/55.74/(14.61) & \textbf{87.96}/85.27/(2.69) \\
\cline{1-5}
\multirow[t]{5}{*}{Resnet34/SVHN} & Imagenet(C) & \textbf{94.34}/93.75/(0.59) & 82.34/\textbf{82.86}/(-0.52) & 89.14/\textbf{90.97}/(-1.83) \\
 & Imagenet(R) & \textbf{93.53}/92.89/(0.64) & 80.67/\textbf{81.44}/(-0.77) & 88.29/\textbf{90.17}/(-1.87) \\
 & LSUN(C) & 88.93/\textbf{92.59}/(-3.67) & 68.54/\textbf{79.82}/(-11.28) & 83.59/\textbf{89.68}/(-6.09) \\
 & LSUN(R) & \textbf{90.69}/90.53/(0.16) & 72.86/\textbf{76.82}/(-3.96) & 84.72/\textbf{88.56}/(-3.84) \\
 & iSUN & 91.23/\textbf{91.50}/(-0.27) & 74.76/\textbf{79.45}/(-4.69) & 85.73/\textbf{89.26}/(-3.54) \\
\cline{1-5}
\bottomrule
\end{tabular}


\end{small}
\end{center}
\end{table}

==> Table_OODV2.tex <==
\begin{table*}
    \caption{Comparison of Quantile-Representations with baseline for OOD Detection. Observe that Quantile-Representations 
    outperform the baseline in all the cases. The entries are represented as \textsc{Baseline}/\textsc{Quantile-Representations}.}
    \label{table:1}
    \begin{center}
    \begin{small}

\begin{tabular}{llllll}
\toprule
 &  &  & AUROC & TNR-TPR95 & Det.Acc \\
Approach & Model/ID & OOD &  &  &  \\
\midrule
\multirow[t]{10}{*}{OneClassSVM} & \multirow[t]{5}{*}{Resnet34/SVHN} & iSUN & 92.28/\textbf{96.13} & 77.43/\textbf{80.15} & 89.77/\textbf{90.65} \\
 &  & LSUN(R) & 91.50/\textbf{95.44} & 74.95/\textbf{77.05} & 89.09/\textbf{89.67} \\
 &  & LSUN(C) & 92.99/\textbf{95.76} & 77.96/\textbf{80.93} & \textbf{90.10}/90.03 \\
 &  & Imagenet(R) & 93.52/\textbf{96.21} & \textbf{79.86}/79.60 & 90.58/\textbf{90.84} \\
 &  & Imagenet(C) & 94.18/\textbf{95.98} & \textbf{81.13}/79.77 & \textbf{91.23}/90.57 \\
\cline{2-6}
 & \multirow[t]{5}{*}{ResNet34/CIFAR10} & iSUN & 90.29/\textbf{93.53} & 41.90/\textbf{61.24} & 84.28/\textbf{87.06} \\
 &  & LSUN(R) & 90.07/\textbf{93.41} & 41.24/\textbf{61.01} & 84.25/\textbf{86.77} \\
 &  & LSUN(C) & 91.74/\textbf{91.79} & 45.87/\textbf{51.96} & \textbf{86.37}/85.77 \\
 &  & Imagenet(R) & 90.33/\textbf{92.33} & 42.18/\textbf{58.95} & 84.21/\textbf{85.47} \\
 &  & Imagenet(C) & 90.96/\textbf{91.44} & 43.95/\textbf{52.08} & \textbf{84.80}/84.58 \\
\cline{1-6} \cline{2-6}
\multirow[t]{10}{*}{LinearSeparability} & \multirow[t]{5}{*}{Resnet34/SVHN} & iSUN & 83.00/\textbf{99.98} & 60.87/\textbf{99.90} & 78.98/\textbf{99.38} \\
 &  & LSUN(R) & 81.90/\textbf{99.98} & 56.34/\textbf{99.97} & 77.76/\textbf{99.47} \\
 &  & LSUN(C) & 80.44/\textbf{99.75} & 52.80/\textbf{99.25} & 75.35/\textbf{97.76} \\
 &  & Imagenet(R) & 80.31/\textbf{99.96} & 57.61/\textbf{99.85} & 77.19/\textbf{99.19} \\
 &  & Imagenet(C) & 81.88/\textbf{99.93} & 61.28/\textbf{99.78} & 78.75/\textbf{98.91} \\
\cline{2-6}
 & \multirow[t]{5}{*}{ResNet34/CIFAR10} & iSUN & 98.73/\textbf{99.94} & 96.06/\textbf{99.88} & 95.75/\textbf{98.92} \\
 &  & LSUN(R) & 98.80/\textbf{99.96} & 96.18/\textbf{99.84} & 95.94/\textbf{99.17} \\
 &  & LSUN(C) & 92.78/\textbf{99.55} & 70.72/\textbf{98.31} & 87.47/\textbf{96.87} \\
 &  & Imagenet(R) & 95.27/\textbf{99.74} & 86.76/\textbf{98.93} & 91.02/\textbf{97.72} \\
 &  & Imagenet(C) & 94.38/\textbf{99.67} & 82.37/\textbf{98.72} & 89.15/\textbf{97.25} \\
\cline{1-6} \cline{2-6}
\bottomrule
\end{tabular}


    \end{small}
    \end{center}
    \end{table*}

==> latexmkrc <==
# This shows how to use the xr package with latexmk.
# John Collins 2023-03-29
#
# The xr package ("a system for eXternal References") is used by a document
# to make references to sections, equations, etc in other external
# documents. 
# The definitions in this file enable latexmk to apply latexmk to
# automatically update an external document whenever its .tex file changes,
# so that the references in the main document stay up to date.

# Notes:
#    1. This version is defined to put the files from the compilations of
#       the external documents into a defined subdirectory, to segregate
#       potentially many generated files from the main document
#       directories. 
#    2. But for latexmk's custom dependency mechanism to be used, as here,
#       the aux file from compilation of a subdocument must be generated in
#       the same directory as the corresponding source .tex file.  So the
#       .aux file is copied.
#    3. It is assumed that the external documents are to be compiled by
#       pdflatex.  This can be changed, of course, by changing the '-pdf'
#       option given to the invoked latexmk to whatever is needed.
#    4. An ideal implementation would also ensure that recompilation of an
#       external document also happens whenever any of its other source
#       files changes.  But this is not done in the present version, and
#       would probably entail either the use of internal latexmk variables
#       or extra enhancements to latexmk.
#    5. The code uses subroutines copy and fileparse that are loaded by
#       latexmk from the Perl packages File::Copy and File::Basename.
#    6. It also uses some not-yet-documented features of latexmk: an array
#       variable @file_not_found and subroutines popd, pushd, and
#       rdb_add_generated. 


#--------------------
# Configurable choices for compilation of external documents

# Subdirectory for output files from compilation of external documents:
$sub_doc_output = 'output-subdoc';

# Options to supply to latexmk for compilation of external documents:
@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

#--------------------

# Add a pattern for xr's log-file message about missing files to latexmk's
# list.  Latexmk's variable @file_not_found is not yet documented.
# This line isn't necessary for v. 4.80 or later of latexmk.
push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne ' ') && ($sub_doc_output ne '.') ) {
               # In this case, .aux file generated by pdflatex isn't in same
               # directory as the .tex file.
               # Therefore:
               # 1. Actual generated aux file must be listed as produced by this
               #    rule, so that latexmk deals with dependencies correctly.
               #    (Problem to overcome: If $sub_dir_output is same as $aux_dir
               #    for the main document, xr may read the .aux file in the
               #    aux_dir rather than the one the cus dep is assumed by latexmk
               #    to produce, which is in the same directory as the .tex source
               #    file for this custom dependency.)
               #    Use not-yet-documented latexmk subroutine rdb_add_generated
               #    to do this:
               # 2. A copy of the .aux file must be in same directory as .tex file
               #    to satisfy latexmk's definition of a custom dependency.
             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}
